Empirical Bayesian Inference using Joint Sparsity

This paper develops a new empirical Bayesian inference algorithm for solving a linear inverse problem given multiple measurement vectors (MMV) of under-sampled and noisy observable data. Specifically, by exploiting the joint sparsity across the multiple measurements in the sparse domain of the underlying signal or image, we construct a new support informed sparsity promoting prior. Several applications can be modeled using this framework, and as a prototypical example we consider reconstructing an image from synthetic aperture radar (SAR) observations using nearby azimuth angles. Our numerical experiments demonstrate that using this new prior not only improves accuracy of the recovery, but also reduces the uncertainty in the posterior when compared to standard sparsity producing priors.

==> blurexperiment.tex <==
As an initial experiment, we directly compare our {support informed sparse prior approach to the hierarchical Gaussian prior (HGP) method} developed in \cite{BardsleyUQ}(Section 4.1). In particular we reconstruct (\ref{eq:true_1D}) from blurred noisy data, which is shown in Figure \ref{fig:bard_comp}(left). The forward model for this problem is given by
 \begin{equation}
 \label{eq:bard_fm}
 [A]_{i,j} = \frac{h}{\sqrt{\pi \gamma^2}}\exp\left(\frac{((i-j)h)^2}{2\gamma^2}\right),
 \end{equation}
where $h = 1/n$ and $\gamma = 0.05$.\footnote{{Since $\gamma$ was not explicitly given in \cite{BardsleyUQ}, we chose it as $.05$ to best match their results.}} The problem is ill-posed, with $\text{cond}(A) \approx 10^{17}$. In \cite{BardsleyUQ}, the standard deviation $\sigma$ of the additive Gaussian white noise (AGWN) is chosen such that {$\sigma = .02 \overline{|x|}$},  which yields $\sigma \approx 0.25$, meaning that only a very small amount of noise is added to each measurement. To simulate additional measurement variability we randomly perturb the parameters used to obtain $J$ independent sparsity vectors in step 4 of Algorithm \ref{alg:SISP}. Further details are found in \cite{VBJS, VBJS_Speckle}. Algorithm \ref{alg:Cross-Validation} yields  $\hat{\lambda} \approx 4.87$. By comparison the hyper-parameter in \cite{BardsleyUQ} was found to be approximately $5.35$.  Figure \ref{fig:bard_comp}(right) displays our resulting MCMC sample mean (\ref{eq:final_approx}) calculated using the proposed posterior in (\ref{eq:PosteriorDensitymask}). Also displayed is $C_{0.05}$, the 95\% credibility bounds. These results should be compared to Figure 4.2(left) in \cite{BardsleyUQ}. We see that with our proposed support informed sparsity prior, the credibility bounds are tighter, indicating reduced uncertainty in the results. Moreover, our resulting MCMC sample mean better resolves areas near discontinuities.  \AG{We also compare the solution in \cite{BardsleyUQ} to the posteriors given by  \eqref{eq:PosteriorDensitylaplace}, \eqref{eq:PosteriorDensityhierarchical}, and \eqref{eq:PosteriorDensitymaskl2}.  Observe that BLAH and since (Fingers crossed) \eqref{eq:PosteriorDensityhierarchical} yields such similar results, we can move on.}


\AG{Things we discussed for this example.
\begin{itemize}
\item  it was impossible to get the right parameters from the Bardsley paper.
\item Their picture was actually much less blurred than ours.
\item If we say it is a comparison, we need to point this out.
\item The other option is to just use this example for blurred data that we make up and just say it doesn't really compare (I still think it's useful to have this example).
\item We will have to take out the $\ell_2$ "Gaussian" figure out of Figure 4.
\end{itemize}
}

\begin{figure}[htb]
\centering
\includegraphics[width=.8\textwidth]{bard_compare.pdf}
\caption{(left) The one-dimensional signal (\ref{eq:true_1D}) and blurred noisy data, as in Figure 4.1 of \cite{BardsleyUQ}. (right) The  MCMC sample mean (\ref{eq:final_approx}) calculated using the proposed posterior in (\ref{eq:PosteriorDensitymask}) with the support informed sparsity prior. Also displayed is $C_{0.05}$, the 95\% credibility bounds. These results should be compared to Figure 4.2(left) in \cite{BardsleyUQ}.}
\label{fig:bard_comp}
\end{figure}



==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage[margin=1in]{geometry}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{url}
\usepackage{color}
\usepackage{framed}
\usepackage{algorithm,algorithmic}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage[normalem]{ulem}
%\usepackage[algo2e]{algorithm2e}
\usepackage[toc,page]{appendix}
\usepackage{amsopn}
%\usepackage{xcolor}
\usepackage[normalem]{ulem}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\newcommand{\AG}{\textcolor{red}}
\newcommand{\TS}{\textcolor{blue}}
\newcommand{\HELP}{\textcolor{cyan}}
\newcommand{\JZ}{\textcolor{green}}

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in} 
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{\AG{Empirical Bayesian Inference Using Joint Sparsity}}{J. Zhang, A. Gelb, and T. Scarnati}
\title{Empirical Bayesian Inference using Joint Sparsity\thanks{Submitted to the editors DATE.
\funding{AG was supported in part by  the NSF grants  DMS \#1502640 and DMS \#1912685,  the Air Force Office of Sponsored Research grant \#FA9550-18-1-0316, and the Office of Naval Research MURI grant \#N00014-20-1-2595.
TS was supported in part by AFOSR LRIR 18RYCOR011. }}}

% Authors: full names plus addresses.
\author{Jiahui Zhang\thanks{Department of Mathematics, Dartmouth College, Hanover, NH 
  (\email{jiahui.zhang.20@dartmouth.edu}%, %\url{http://www.imag.com/\string~ddoe/}
  ).}
\and Anne Gelb\thanks{Department of Mathematics, Dartmouth College, Hanover, NH
  (\email{annegelb@math.dartmouth.edu}).}
\and Theresa Scarnati\thanks{Air Force Research Laboratory, Wright-Patterson AFB, USA.
  (\email{theresa.scarnati.1@us.af.mil}).}}



\DeclareMathOperator{\diag}{diag}

\newcommand*{\bbR}{\mathbb{R}}
\newcommand*{\supp}{\mathrm{supp}}
%\newcommand*{\argmin}[1]{{\underset{#1}{\operatorname{argmin}}}}
%\newcommand*{\argmax}[1]{{\underset{#1}{\operatorname{argmax}}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\bes}[1]{\begin{equation*} #1 \end{equation*}}
\newcommand*{\nm}[1]{{\left\|#1\right \|}}
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

